Hutch++: Optimal Stochastic Trace Estimation

We study the problem of estimating the trace of a matrix $A$ that can only be accessed through matrix-vector multiplication. We introduce a new randomized algorithm, Hutch++, which computes a $(1 \pm \epsilon)$ approximation to $tr(A)$ for any positive semidefinite (PSD) $A$ using just $O(1/\epsilon)$ matrix-vector products. This improves on the ubiquitous Hutchinson's estimator, which requires $O(1/\epsilon^2)$ matrix-vector products. Our approach is based on a simple technique for reducing the variance of Hutchinson's estimator using a low-rank approximation step, and is easy to implement and analyze. Moreover, we prove that, up to a logarithmic factor, the complexity of Hutch++ is optimal amongst all matrix-vector query algorithms, even when queries can be chosen adaptively. We show that it significantly outperforms Hutchinson's method in experiments. While our theory mainly requires $A$ to be positive semidefinite, we provide generalized guarantees for general square matrices, and show empirical gains in such applications.

==> adaptive-estimation-old.tex <==
\newpage

\section{An Adaptive Estimator using Rank-\texorpdfstring{\(k\)}{k} Projections}

The variance of Hutchinson estimator is fundamentally tied to the Frobenius norm of the target matrix.
In \appendixref{hutch-frob}, we prove a close analogue of Theorem 5 in \cite{DBLP:journals/corr/abs-2005-10009}, making the relationship between the Hutchinson estimator the the Frobenius norm more explicit:
\begin{lemma}
\label{lem:hutch}
Let \(\mA\in\bbR^{d \times d}\) and \(\ell\in\bbN\).
Then, with probability \((1-\delta)\), the \(\ell\)-sample Hutchinson estimate for \(\trace(\mA)\) satisfies
\[
	\abs{\trace(\mA) - \hutch_\ell(\mA)} \leq O\left(\sqrt{\tsfrac{\log(\nicefrac1\delta)}{\ell}}\right) \normof\mA_F
\]
Or, equivalently,
\[
	\trace(\mA) \in \hutch_\ell(\mA) \pm O\left(\sqrt{\tsfrac{\log(\nicefrac1\delta)}{\ell}}\right) \normof\mA_F
\]
\end{lemma}

Since \(\normof{\mA}_F \leq \trace(\mA)\) for PSD matrices, this implies \(\abs{\trace(\mA) - \hutch_\ell(\mA)} \leq O\left(\sqrt{\frac{\log(\nicefrac1\delta)}{\ell}}\right) \trace(\mA)\), proving that \(\ell=O(\frac{1}{\eps^2})\) queries suffice to get a \((1\pm\eps)\) relative error approximation to \(\trace(\mA)\).
This analysis for the Hutchinson estimator is asymptotically tight \cite{DBLP:conf/icalp/WimmerWZ14}.
Also, this suggests that the worst-case input matrices for the Hutchinson estimator have \(\trace(\mA)\approx\normof\mA_F\).

Now recall that for PSD matrices with eigenvalues \(\vlambda = [\lambda_1,\ldots,\lambda_d]^\intercal\), \(\trace(\mA)=\normof{\vlambda}_1\) and \(\normof\mA_F = \normof\vlambda_2\).
So, if we know that \(\trace(\mA) \approx \normof\mA_F\), then \(\normof\vlambda_1 \approx \normof\vlambda_2\), which in turn implies that most of the mass of \vlambda is contained in a small number of its elements.
In other words, \(\normof\vlambda_1 = \trace(\mA)\) is well described by the top few eigenvalues.
Is then relevant that there exists many algorithms that can efficiently isolate the top few eigenvalues of a matrix\cite{DBLP:journals/corr/abs-2004-08434,...}.

The worst case input matrices for the Hutchinson estimator have this structure where a few eigenvalues approximate the trace very well, so we propose algorithms that work in two steps:
\begin{enumerate}
	\item Estimate the top few eigenvalues \mA using tools from the sketching and streaming literature
	\item Estimate the sum of the remaining smaller eigenvalues using the Hutchinson Estimator
\end{enumerate}

The first algorithm we propose is an adaptive algorithm that uses low-rank projection matrices, which we call \emph{AdaHutch}:
\begin{algorithm}[H]
	\caption{Adaptive Hutchinson}
	\label{alg:adahutch2}
	% 
	{\bfseries input}: PSD Matrix \(\mA\in\bbR^{d \times d}\) with Matrix-Vector query access. Amounts of queries \(k\), \(\ell\).\\
	% 
	{\bfseries output}: Approximate Trace of \mA.
	%
	% \phantom{aaaaaaaaaaaaaaaaaaaaaaaaaaaaaaa}
	% \vspace{-\baselineskip}
	% 
\begin{algorithmic}[1]
	\STATE Sample \(\mS \in \bbR^{d \times \frac k2}\) and \(\mG\in\bbR^{d \times \ell}\) with iid \(\cN(0,1)\) entries
	\STATE Compute the economic QR Decomposition \(\mQ = \text{qr}(\mA\mS) \in \bbR^{d \times \frac k2}\)
	\STATE Compute the projection matrix \(\mP = \mQ\mQ^\intercal \in \bbR^{d \times d}\)
	\STATE {\bfseries return} \(\trace(\mA) \approx \trace(\mQ^\intercal\mA\mQ) + \frac{1}{\ell}\trace(\mG^\intercal(\eye-\mP)\mA(\eye-\mP)\mG)\)
\end{algorithmic}
\end{algorithm}

Intuitively, think of \mQ as the column space for the first \(O(k)\) eigenvectors, as found by a single step of subspace iteration.
Then \(\trace(\mQ^\intercal\mA\mQ)\) is the sum of the first \(O(k)\) eigenvalues.
Further, \(\eye-\mP\) projects \mA away from those first \(O(k)\) eigenvectors, so that \(\frac{1}{\ell}\trace(\mG^\intercal(\eye-\mP)\mA(\eye-\mP)\mG)\) is the Hutchinson estimate for all the smaller eigenvalues.
Formally, we can prove the following:

\begin{theorem}
\label{thm:adahutch2}
Let \(\mA\in\bbR^{d \times d}\) be an SPD matrix, fix error parameter \(\eps > 0\) and failure probability \(\delta \in(0,1)\).
Then, running \algorithmref{adahutch} with \(k=O(\frac1\eps + \log(\nicefrac1\delta))\) and \(\ell=O(\frac{\log(\nicefrac1\delta)}\eps)\) returns a \((1\pm\eps)\) relative error approximation to \(\trace(\mA)\) with probability \(1-\delta\).
\end{theorem}
Since \algorithmref{adahutch} uses exactly \(k+\ell\) matrix-vector queries, this process uses \(O(\frac{\log(\nicefrac1\delta)}{\eps})\) matrix-vector queries.
\begin{proof}
Let \(\mP\) be any projection matrix that has rank \(O(k)\) and satisfies \(\normof{\mA-\mP\mA}_F^2 \leq 2 \normof{\mA-\mA_k}_F^2\), where \(\mA_k\) is the best rank-\(k\) approximation to \mA.
Let orthogonal \(\mQ \in \bbR^{d \times k}\) span the column space of \mP.
Using the linearity of trace, the fact that \(\mP=\mP^2\), \((\eye-\mP)=(\eye-\mP)^2\), and the cyclic property of trace, we find
\begin{align*}
	\trace(\mA)
	&= \trace(\mP\mA) + \trace((\eye-\mP)\mA) \\
	&= \trace(\mP\mP\mA) + \trace((\eye-\mP)(\eye-\mP)\mA) \\
	&= \trace(\mP\mA\mP) + \trace((\eye-\mP)\mA(\eye-\mP)) \\
\end{align*}
Note that \(\mP\mA\mP\) is the projection of \mA onto its top eigenvectors, while \((\eye-\mP)\mA(\eye-\mP)\) is the projection away from those same directions.
Since \(\mP=\mQ\mQ^\intercal\),
\[	
	\trace(\mP\mA\mP)
	= \trace(\mQ\mQ^\intercal\mA\mQ\mQ^\intercal)
	= \trace(\mQ^\intercal\mA\mQ\mQ^\intercal\mQ)
	= \trace(\mQ^\intercal\mA\mQ)
\]
we transform to the \mQ matrix because it would take \(d\) matrix-vector products to compute \(\mA\mP\), but only takes \(O(k)\) matrix-vector products to compute \(\mA\mQ\).
Returning to \(\trace(\mA)\), and recalling \lemmaref{hutch},
\begin{align*}
	\trace(\mA)
	&= \trace(\mP\mA\mP) + \trace((\eye-\mP)\mA(\eye-\mP)) \\
	&= \trace(\mQ^\intercal\mA\mQ) + \trace((\eye-\mP)\mA(\eye-\mP)) \\
	&\in \trace(\mQ^\intercal\mA\mQ) + \hutch_\ell((\eye-\mP)\mA(\eye-\mP)) \pm \tilde O(\tsfrac{1}{\sqrt\ell})\normof{(\eye-\mP)\mA(\eye-\mP)}_F^2
\end{align*}
Where \(\hutch_\ell(\mM)\) is the result of running the Hutchinson estimator on \mM with \(\ell\) queries.
All we need to do now is bound the lingering Frobenius norm.
By the submultiplicativity of the Frobenius norm, and since \(\normof{\eye-\mP}_2 = 1\),
\[
	\normof{(\eye-\mP)\mA(\eye-\mP)}_F \leq \normof{\mA - \mP\mA}_F \cdot \normof{\eye-\mP}_2 \leq 2 \normof{\mA-\mA_k}_F
\]
where the last inequality uses our guarantee on \mP.
Next, recall that if \mA has eigenvalues \(\lambda_1,\ldots,\lambda_d\), then \(\mA-\mA_k\) has eigenvalues \(\lambda_{k+1},\ldots,\lambda_d\).
So,
\[
	\normof{\mA-\mA_k}_F^2 = \sum_{i=k+1}^d \lambda_i^2 \leq \lambda_{k+1} \sum_{i=k+1}^d \lambda_i \leq \frac1k \trace(\mA) \sum_{i=k+1}^d \lambda_i \leq \frac1k (\trace(\mA))^2
\]
where the second inequality uses the relationship \(\lambda_{k+1} \leq \frac1k \sum_{i=1}^k \lambda_i \leq \frac1k \trace(\mA)\).
With this bound, we conclude
\[
	\normof{(\eye-\mP)\mA(\eye-\mP)}_F \leq \sqrt{\frac2k}\trace(\mA)
\]
Intuitively, thinking of the Frobenius norm as the standard deviation of the Hutchinson estimator, this inequality shows how projecting off the top \(O(k)\) directions tightens the estimator's predictions.
Returning to our bound on \(\trace(\mA)\),
\begin{align*}
	\trace(\mA)
	&\in \trace(\mQ^\intercal\mA\mQ) + \hutch_\ell((\eye-\mP)\mA(\eye-\mP)) \pm \tilde O(\tsfrac{1}{\sqrt\ell})\normof{(\eye-\mP)\mA(\eye-\mP)}_F^2 \\
	&\subseteq \trace(\mQ^\intercal\mA\mQ) + \hutch_\ell((\eye-\mP)\mA(\eye-\mP)) \pm \tilde O(\tsfrac{1}{\sqrt\ell})\sqrt{\tsfrac2k}\trace(\mA)
\end{align*}
Rearranging the above, we find
\[
	\trace(\mQ^\intercal\mA\mQ) + \hutch_\ell((\eye-\mP)\mA(\eye-\mP)) \in \left(1 \pm \tilde O(\tsfrac1{\sqrt{k\ell}})\right)\trace(\mA)
\]
If we take \(k = O(\frac1\eps)\) and \(\ell = O(\frac{\log(\nicefrac1\delta)}{\eps})\), then this implies \((1+\eps)\)relative error.

All we have to show now is show that the \mP matrix in \algorithmref{adahutch} satisfies \(\normof{\mA-\mP\mA}_F \leq 2 \normof{\mA-\mA_k}_F\).
Noting that \mP is the best Rank-\(O(k)\) projection matrix for \(\mA\mS\), Corollary 7 and Claim 1 from \cite{DBLP:journals/corr/abs-2004-08434} tell us that \(\normof{\mA-\mP\mA}_F^2 \leq 2 \normof{\mA-\mA_k}_F^2\), so long as \mS has \(\Omega(k+\log(\nicefrac1\delta)) = \Omega(\frac1\eps + \log(\nicefrac1\delta))\) samples.
Further, \mQ is clearly an orthogonal basis for the column space of \mP.
\end{proof}

% \Raph{Ideas for next draft:
% \begin{itemize}
% 	\item Make \mP and \mQ inputs to adahutch
% 	\begin{itemize}
% 		\item \theoremref{adahutch} assumes that \(\normof{\mA-\mP\mA}_F \leq 2 \normof{\mA-\mA_{k/2}}_F\). Note that subscript gotta be \(\frac k2\) since \(\frac k2\) queries are needed for both the sketch and the trace.
% 		\item The QR algo for \mP and \mQ should be a seperate algo
% 		\item \theoremref{adahutch} should be really short. That makes it look clean.
% 	\end{itemize}
% 	\item \(\normof{\mA-\mA_k} \leq \sqrt{\frac2k} \trace(\mA)\) should be an outside lemma before the proof. It fits well with the preceeding intuitions, and lets us avoid the weird \(\frac k2\) notation
% 	\item adahutch should take in 1 parameter for number of queries, and it should be a factor of 3. Let \(k\) be the number of queries and \(\ell=\frac k3\in\bbN\) be the size of each query.
% \end{itemize}}



==> adaptive-estimation.tex <==
\section{Adaptive Trace Estimation with low-rank Projections}
The variance of the Hutchinson estimator is fundamentally tied to the Frobenius norm of the target matrix.
In \appendixref{hutch-frob}, we prove an analogue of Theorem 5 in \cite{DBLP:journals/corr/abs-2005-10009}, which makes the relationship between the Hutchinson estimator and the Frobenius norm explicit:
\begin{lemma}
\label{lem:hutch-frob}
Let \(\mA\in\bbR^{d \times d}\), \(\ell\in\bbN\), and \(\delta\in (0, 1)\).
Then, with probability \(1-\delta\), the \(\ell\)-query Hutchinson estimate of \(\trace(\mA)\) satisfies
\[
	\abs{\trace(\mA) - \hutch_\ell(\mA)} \leq O\left(\sqrt{\frac{\log(\nicefrac1\delta)}{\ell}}\right)\normof\mA_F
\]
We will often write \(\tilde O(\frac{1}{\sqrt \ell})\) to hide the logarithmic dependence on \(\delta\).
\end{lemma}
Since \(\normof\mA_F \leq \trace(\mA)\) for PSD matrices, \lemmaref{hutch-frob} implies \(\abs{\trace(\mA)-\hutch_\ell(\mA)} \leq \tilde O(\frac1{\sqrt\ell})\trace(\mA)\).
So, \(\ell=\tilde O(\frac1{\eps^2})\) queries suffice to get a \((1\pm\eps)\) relative error approximation to \(\trace(\mA)\).
While this analysis is tight for the Hutchinson estimator \cite{DBLP:conf/icalp/WimmerWZ14}, it also suggests that the Hutchinson estimator only needs \(\tilde O(\frac1{\eps^2})\) samples in the hard case when \(\trace(\mA)\approx\normof\mA_F\).

Let \(\vlambda = \bmat{\lambda_1 & \ldots & \lambda_d}^\intercal\) be the eigenvalues of \mA, so that \(\trace(\mA)=\normof\vlambda_1\) and \(\normof\mA_F = \normof\vlambda_2\).
So, if we know that \(\trace(\mA)\approx\normof\mA_F\), then \(\normof\vlambda_1\approx\normof\vlambda_2\), which in turn implies that most of the mass of \vlambda is concentrated in a small number of its indices.\footnote{For instance, a nonzero vector \vx has \(\normof\vx_1 = \normof\vx_2\) if and only if \vx has exactly one nonzero entry.}
In other words, \(\normof\vlambda_1=\trace(\mA)\) is well described by the top few eigenvalues.
% Let \(\vlambda=\bmat{\lambda_1 & \ldots & \lambda_d}^\intercal\) be the eigenvalues of \mA, so that \(\trace(\mA) = \normof\vlambda_1\) and \(\normof\mA_F = \normof\vlambda_2\).
% If \mA is a hard input matrix for the Hutchinson estimator, we know that \(\trace(\mA)\approx\normof\mA_F\), and so \(\normof\vlambda_1\approx\normof\vlambda_2\).
% Further, we know that the L1 and L2 norms of a vector are only close when that vector is mostly concentrated in a small number of indices\footnote{For instance, \(\normof{\vx}_1 = \normof\vx_2\) if and only if \vx has at most one nonzero entry}.
% In our case, this means that if \mA is a hard input for the Hutchinson estimator, then most of its trace is concentrated in the top few eigenvalues.
Here is a technical lemma that reinforces this intuition:
\begin{lemma}
\label{lem:low-rank-frob-trace}
Let \(\mA_k\) be the best rank-\(k\) approximation to PSD matrix \mA.
Then,
\[
	\normof{\mA - \mA_k}_F \leq \frac{1}{\sqrt k}\trace(\mA)
\]
\end{lemma}
\begin{proof}
Note that \(\lambda_{k+1} \leq \frac1k \sum_{i=1}^k \lambda_i \leq \frac1k \trace(\mA)\), so that
\[
	\normof{\mA-\mA_k}_F^2 = \sum_{i=k+1}^d \lambda_i^2 \leq \lambda_{k+1} \sum_{i=k+1}^d \lambda_i \leq \left(\frac1k\trace(\mA)\right)\sum_{i=k+1}^d \lambda_i \leq \frac1k (\trace(\mA))^2
\]
\end{proof}
Intuitively, if \(\normof\mA_F \approx \trace(\mA)\), then \lemmaref{low-rank-frob-trace} ensures us that \(\normof{\mA_k}_F \gtrapprox \sqrt{1-\frac1k}\trace(\mA)\)\footnote{To see this, rearrange the expression \((\trace(\mA))^2=\normof{\mA}_F^2 = \normof{\mA_k}_F^2 + \normof{\mA-\mA_k}_F^2 \leq \normof{\mA_k}_F^2 + \frac{1}{k}\trace(\mA)\)}.
Combined with the fact that \(\sum_{i=1}^k \lambda_i = \trace(\mA_k) \geq \normof{\mA_k}_F\), we find \(\sum_{i=1}^k \lambda_i \gtrapprox \sqrt{1-\frac1k} \trace(\mA)\), which means that the top \(k\) eigenvalues of represent almost the entire trace of \mA.
In short:
\begin{center}
	\emph{
	If \(\mA\) is a hard input for the Hutchinson estimator,\\then the top few eigenvalues of \mA approximate the trace of \mA very well.
	\\
	\vspace{1em}
	If \(\mA\) is an easy input for the Hutchinson estimator,\\then use the Hutchinson estimator
	}
\end{center}
However, in order to avoid testing if \mA is an easy or hard input, we will always do both: all algorithms we propose start by using streaming or sketching tools to estimate the sum of the first few eigenvalues, and then use Hutchinson to estimate the rest.
% However, in order to avoid testing if \mA is an easy or hard input, we will always do both: all the algorithms we propose start by estimating the sum of the first few eigenvalues, and then use Hutchinson to estimate the sum of the rest of the eigenvalues.
The Adaptive Hutchinson Estimator, or \emph{AdaHutch}, is the first estimator we propose and follows this pattern:
\begin{theorem}
\label{thm:adahutch}
Let \(\mP\in\bbR^{d \times d}\) be a rank-\(O(k)\) projection matrix such that \(\normof{\mA-\mP\mA}_F \leq 2 \normof{\mA-\mA_k}_F\).
Let \(\mQ\in\bbR^{d \times O(k)}\) be an orthogonal matrix that spans the column space of \mP.
Then let
\[
	\adahutch_{k,\ell}(\mA) \defeq \trace(\mQ^\intercal\mA\mQ) + \hutch_\ell((\eye-\mP)\mA(\eye-\mP))
\]
which can be evaluated with \(\ell + O(k)\) matrix-vector queries to \mA.
If \(\delta\in (0, 1)\), then with probability \(1-\delta\), we have
\[
	\abs{\adahutch_{k,\ell}(\mA) - \trace(\mA)} \leq O\big( {\textstyle \sqrt{\frac{\log(\nicefrac1\delta)}{k\ell}}}\big) \trace(\mA)
\]
In particular, if \(k = \ell = O(\frac{\sqrt{\log(\nicefrac1\delta)}}{\eps})\), then \(\adahutch_{k,\ell}\) uses \(O(\frac{\sqrt{\log(\nicefrac1\delta)}}{\eps})\) matrix-vector queries to get a \((1\pm\eps)\) relative error guarantee.
\end{theorem}
In the \(\adahutch_{k,\ell}\) definition, \(\trace(\mQ^\intercal\mA\mQ)\) approximates the trace of the top \(k\) eigenvalues, while the \(\hutch_\ell\) term approximates the trace of the rest of the eigenvalues.
Note that Corollary 7 and Claim 1 from \cite{DBLP:journals/corr/abs-2004-08434} prove that a single step of subspace iteration suffices to find such a matrix \mP, leading to the following algorithm for approximating the trace of \mA:

\begin{algorithm}[H]
	\caption{Adaptive Hutchinson}
	\label{alg:adahutch}
	% 
	{\bfseries input}: Matrix-Vector oracle to PSD Matrix \(\mA\in\bbR^{d \times d}\). Number of queries \(k\) and \(\ell\) (\(k\) is even). \\
	% 
	{\bfseries output}: Approximate Trace of \mA
	% 
	% \phantom{aaaaaaaaaaaaaaaaaaaaaaaaaaaaaaa}
	% \vspace{-\baselineskip}
	% 
\begin{algorithmic}[1]
	\STATE Sample \(\mS\in\bbR^{d \times \frac k2}\) and \(\mG\in\bbR^{d \times \ell}\) with \iid \(\cN(0,1)\) entries
	\STATE Compute QR matrix \(\mQ = \text{qr}(\mA\mS) \in \bbR^{d \times \frac k2}\)
	\STATE Compute \(\mP = \mQ\mQ^\intercal\)
	\STATE {\bfseries return} \(\adahutch_{k,\ell} = \trace(\mQ^\intercal\mA\mQ) + \frac1\ell \trace(\mG^\intercal(\eye-\mP)\mA(\eye-\mP)\mG)\)
\end{algorithmic}
\end{algorithm}

\begin{corollary}
Since Corollary 7 from \cite{DBLP:journals/corr/abs-2004-08434} requires \(O(k + \log(\nicefrac1\delta))\) matrix-vector queries to ensure \(\normof{\mA-\mP\mA}_F\leq2\normof{\mA-\mA_k}_F\), \algorithmref{adahutch} requires \(O(\frac{\sqrt{\log(\nicefrac1\delta)}}\eps + \log(\nicefrac1\delta)) = \tilde O(\frac1\eps)\) matrix-vector queries for a \((1\pm\eps)\) relative error approximation.
\end{corollary}

\begin{proof}[Proof of \theoremref{adahutch}]
Recall that since \mP is a projection matrix, \(\mP=\mP\mP\) and \((\eye-\mP)=(\eye-\mP)(\eye-\mP)\).
Then,
\begin{align*}
	\trace(\mA)
	&= \trace(\mP\mA) + \trace( (\eye-\mP)\mA) \\
	&= \trace(\mP\mP\mA) + \trace((\eye-\mP)(\eye-\mP)\mA) \\
	&= \trace(\mP\mA\mP) + \trace((\eye-\mP)\mA(\eye-\mP))
\end{align*}
where the last line uses the cyclic property of trace.
Next, recall that \(\mP=\mQ\mQ^\intercal\), so that
\[
	\trace(\mP\mA\mP)
	= \trace(\mQ\mQ^\intercal\mA\mQ\mQ^\intercal)
	= \trace(\mQ^\intercal\mA\mQ\mQ^\intercal\mQ)
	= \trace(\mQ^\intercal\mA\mQ)
\]
and therefore
\[
	\trace(\mA)
	= \trace{\mQ^\intercal\mA\mQ} + \trace((\eye-\mP)\mA(\eye-\mP)) \\
\]
So, by applying \lemmaref{hutch-frob} on the matrix \((\eye-\mP)\mA(\eye-\mP)\), we know that
\begin{align*}
	\abs{\adahutch_{k,\ell}(\mA) - \trace(\mA)}
	% &= \abslr{\trace((\eye-\mP)\mA(\eye-\mP)) - \hutch_\ell( (\eye-\mP)\mA(\eye-\mP))} \\
	&\leq \tilde O(\tsfrac1{\sqrt \ell}) \normof{(\eye-\mP)\mA(\eye-\mP)}_F
\end{align*}
To complete the theorem, we just need to show that \(\normof{(\eye-\mP)\mA(\eye-\mP)}_F \leq O(\frac1{\sqrt k}) \trace(\mA)\).
By submultiplicativity, the fact that \(\normof{\eye-\mP}_2 = 1\), and our assumption on \mP,
\[
	\normof{(\eye-\mP)\mA(\eye-\mP)}_F \leq \normof{\mA-\mP\mA}_F \cdot \normof{\eye-\mP}_2 \leq 2\normof{\mA-\mA_k}_F
\]
And, lastly, by \lemmaref{low-rank-frob-trace}, \(\normof{\mA-\mA_k}_F \leq \frac{1}{\sqrt k} \trace(\mA)\), completing the proof.
\end{proof}



==> app-lower-bounds.tex <==
\section{Bounding \texorpdfstring{\(D_{KL}(\chi_{n}^2\|\chi_{n+1}^2)\)}{the DKL of Chi-Squared Variables}}
\label{app:dkl-bound}
\begin{lemma}
For any \(n\in\bbN\), \(D_{KL}(\chi_n^2\|\chi_{n+1}^2) \leq \frac1n\).
\end{lemma}
\begin{proof}
Note that \(\E_{t\sim\chi_n^2}[t] = n\), and \(\E_{t\sim\chi_n^2}[\ln(t)] = \ln(2) + \psi(\frac n2)\) where \(\psi\) is the digamma function \cite{pav2015moments}.
Denoting the differential entropy of a chi-squared variable as \(h(\chi_n^2)\),
\begin{align*}
	D_{KL}(\chi_n^2 \| \chi_\ell^2)
	&= - h(\chi_n^2) - \E_{t\sim\chi_n^2}\left[\ln(p_\ell(t))\right] \\
	&= - h(\chi_n^2) - \E_{t\sim\chi_n^2}\left[\ln(2^{-\nicefrac n2}(\Gamma(\tsfrac n2))^{-1}t^{(\frac\ell2 - 1)}e^{-\frac t2})\right] \\
	&= - h(\chi_n^2) + \frac{\ln(2)}2 \ell + \ln(\Gamma(\tsfrac n2)) - (\tsfrac \ell2 - 1)\E_{t\sim\chi_n^2}[\ln(t)] + \frac12 \E_{t\sim\chi_n^2}\left[t\right] \\
	&= - h(\chi_n^2) + \frac{\ln(2)}2 \ell + \ln(\Gamma(\tsfrac n2)) - (\tsfrac \ell2 - 1)(\ln(2) + \psi(\tsfrac n2)) + \tsfrac n2 \\
	&= - h(\chi_n^2) + \ln(\Gamma(\tsfrac n2)) + \ln(2) - (\tsfrac \ell2 - 1)\psi(\tsfrac n2) + \tsfrac n2.
\end{align*}
Substituting in \(h(\chi_n^2) = \frac n2 + \ln(\Gamma(\frac n2)) + \ln(2) + (1 - \frac n2) \psi(\frac n2)\) from \cite{lazo1978entropy} and then simplifying, we get
\[
	D_{KL}(\chi_n^2 \| \chi_\ell^2)
	=
	\ln(\tsfrac{\Gamma(\nicefrac\ell2)}{\Gamma(\nicefrac n2)}) + \tsfrac{n-\ell}2 \psi (\tsfrac n2)
\]
And so, when \(\ell = n+1\), \(D_{KL}(\chi_n^2 \| \chi_{n+1}^2) = \ln(\tsfrac{\Gamma(\nicefrac{n+1}2)}{\Gamma(\nicefrac n2)}) - \tsfrac{1}2 \psi (\tsfrac n2)\).
We now import two useful results.
First, Equation 6 of \cite{wendel1948note} tells us that for any \(x\geq0\) and \(a\in(0,1)\), \(\frac{\Gamma(x+1)}{\Gamma(x+a)} \leq (x+a)^{1-a}\).
With \(x=\frac{n-1}{2}\) and \(a = \frac12\), this bound tells us that
\[
	\ln(\tsfrac{\Gamma(\nicefrac{n+1}2)}{\Gamma(\nicefrac n2)})
	= \ln(\tsfrac{\Gamma(\frac{n-1}{2} + 1)}{\Gamma(\frac{n-1}{2}+\frac12)})
	\leq \ln((\tsfrac{n-1}{2} + \tsfrac12)^{1-\frac12})
	= \frac12 \ln(\tsfrac n2).
\]
Second, Equation \(2.2\) of \cite{DBLP:journals/moc/Alzer97} tells us that for any \(x \geq 0\), \(\psi(x) > \ln(x) - \frac1x\).
With \(x=\frac n2\), this tells us that
\[
	\tsfrac{1}2 \psi (\tsfrac n2)
	> \frac12(\ln(\tsfrac n2) - \tsfrac 2n) = \frac12\ln(\tsfrac n2) - \frac1n.
\]
And altogether we get
\[
	D_{KL}(\chi_n^2 \| \chi_{n+1}^2) < \frac12 \ln(\tsfrac n2) - \left(\frac12\ln(\tsfrac n2) - \frac1n\right) = \frac1n.
\]


\end{proof}


==> lower-bound.tex <==
% !TEX root = ./hutchplusplus.tex

\section{Lower Bound: Non-Adaptive Estimators Require \texorpdfstring{\(\Omega(\frac{1}{\eps})\)}{1 / eps} Queries}
\label{sec:lower_bound}
A natural question is if the $O(1/\epsilon)$ matrix vector multiplication query bound of \theoremref{intro_thm} and \theoremref{hutchna} is tight.
%Since \hutchpp converges faster than the prior rates, which were all \(\tilde O(\frac1{\eps^2})\), we are left with a natural question: Is it possible to converge with fewer than \(\tilde O(\frac1\eps)\) Matrix-Vector queries?
We prove that it is for all algorithms that perform non-adaptive queries like \hutchppna.
%We prove that this is not possible in non-adaptive setting, where the algorithm must declare all their queries before seeing any response vectors.

%Recall the intuition we provided in \sectionref{upper_bound_proof}.
%If the eigenvalues of \mA are concentrated in very few entries, then sketching can recover \(\trace(\mA)\) very quickly.
%If the eigenvalues of \mA are evenly spread out, then \(\normof\mA_F \ll \trace(\mA)\),\footnote{Suppose \(\vlambda\in\bbR^d\) is the all-ones vector. Then \(\normof\mA_F=\normof\vlambda_2 = \sqrt d \ll d = \normof\vlambda_1 = \trace(\mA)\).} so the Hutchinson estimator can recover \(\trace(\mA)\) very quickly.
%A hard trace estimation problem should lie somewhere between these two extremes.

%In particular, note that \hutchpp and \hutchppna both project off \(O(\frac1\eps)\) top eigendirections and then estimate the trace of the remainder.
%So, 
We consider the problem of {distinguishing random rotations of two diagonal matrices}: one with \(\frac1\eps\) entries equal to $1$, and the rest $0$  and the second with \(\frac1\eps+1\) entries equal to $1$, and the rest $0$.
Since \(\frac1\eps+1 = (1+\eps)\frac1\eps\), a trace estimator with that achieves relative error \(1 \pm \eps\) can distinguish these matrices. We prove that this requires \(\Omega(\frac1\eps)\) matrix-vector multiplication queries.
Formally,

\begin{problem}
\label{prob:trace-style}
Fix \(d\in\bbN\) and \(\eps < 1\) such that \(n\defeq\frac1\eps\in\bbN\) and \(n < d\).
Let \(\mD_1 \defeq \spmat{\eye_n & \\ & \mat0_{d-n}}\) and \(\mD_2 \defeq \spmat{\eye_{n+1} & \\ & \mat0_{d-(n+1)}}\).
Nature selects \(\mD=\mD_1\) or \(\mD=\mD_2\) with equal probability, samples \(\mG\in\bbR^{d \times d}\) with \iid \(\cN(0,1)\) entries, and computes \(\mA = \mG^T\mD\mG\).
The user fixes a query matrix \(\mU\in\bbR^{d \times m}\), observes \(\mA\mU\in\bbR^{d \times m}\) and guesses if \(\mD=\mD_1\) or \(\mD=\mD_2\).
\end{problem}
We first show that a relative error trace estimation algorithm using non-adaptive matrix-vector multiplication queries suffices to solve \problemref{trace-style}.
%
%Intuitively, a trace estimator should be able to solve \problemref{trace-style} efficiently, since \(\frac1d\trace(\mG^T\mD\mG) \approx \trace(\mD)\).
%So, since \(\mD_2\) has \(1+\eps\) times the trace of \(\mD_1\), a trace estimator should be able to distinguish the two matrices.
%Formally,
\begin{lemma}
\label{lem:lower-bound-trace-style}
Suppose an algorithm \cA uses \(m\) non-adaptive matrix-vector multiplication queries to estimate the trace of a matrix to relative error \(1 \pm \frac\eps6\) and succeeds with probability at least \(\frac34\).
Then, for large enough dimension \(d\), \cA can be used to solve \problemref{trace-style} with probability at least \(\frac23\).% and $m$ queries.
\end{lemma}
\begin{proof}
%First we show that the trace of \(\mA = \mG^T\mD\mG\) is close to the trace of \(\mD\) with high probability when the dimension $d$ is large enough. 
Note that $\tr(\mA) = \tr(\mG^T\mD \mG)$ is a scaled Hutchinson estimate for $\tr(\mD)$:
$\trace(\mG^T\mD_1\mG) = d \cdot \hutch_d(\mD)$. Via \lemmaref{hutch-frob}, for large enough $d$ we thus have with probability $\ge \frac{11}{12}$:
%Theorem 3 from \cite{Roosta-KhorasaniAscher:2015} says that for PSD matrices \mA, \(\abs{\hutch_\ell(\mA)-\trace(\mA)}\leq(1+\eps)\trace(\mA)\) if \(\ell \geq \frac8{\eps^2}\log(\nicefrac2\delta)\).
%So, with a union bound, we find that with probability \(\frac{11}{12}\),
\[
	\frac1d\trace(\mG^T\mD_1\mG) \leq \left (1+\frac{\epsilon}{6}\right )\trace(\mD_1)
	\hspace{0.75cm}
	\text{and}
	\hspace{0.75cm}
	\frac1d\trace(\mG^T\mD_2\mG) \geq \left(1-\frac{\epsilon}{6}\right )\trace(\mD_2).
\]
Additionally, with probability \(\frac34\), \cA computes an approximation $Z$ with $(1-\frac\eps6) \tr(\mA) \le Z \le (1+\frac\eps6) \tr(\mA)$.
% an approximate trace \(\tilde\trace(\mA)\) with relative error at most \(\frac\eps3\).
By the union bound, all the above events happen with probability $\ge \frac23$.
If \(\mD=\mD_1\):
\[
	Z \leq (1+\tsfrac\eps6) \tr(\mA) \le (1+\tsfrac\eps6)^2 \cdot d \cdot \trace(\mD_1).% < (1+\epsilon) \cdot d \cdot \frac{1}{\epsilon} = \frac{d}{\epsilon} + d.
\]
On the other hand, if \(\mD=\mD_2\), since $\tr(\mD_2) = (1+\eps) \tr(\mD_1)$:
%Since \(\trace(\mD_2)=(1+\eps)\trace(\mD_1)\), if \(\mD=\mD_2\), we have
\[
	Z \ge (1-\tsfrac\eps6) \tr(\mA) \ge (1-\tsfrac\eps6)^2 \cdot d \cdot \trace(\mD_2) =  (1-\tsfrac\eps6)^2 \cdot (1+\eps) \cdot d \cdot \trace(\mD_1) .%> (1-\epsilon) \cdot d \cdot \left (\frac{1}{\epsilon}+1 \right ) = \frac{d}{\epsilon} + d.
\]
We can check that  $(1-\tsfrac\eps6)^2 \cdot (1+\eps) > (1+\tsfrac\eps6)^2$ for all $\epsilon \in (0,1]$. Thus, checking if  $Z > (1+\tsfrac\eps6)^2 \cdot d \cdot \trace(\mD_1)$ suffices to distinguish whether $\mD = \mD_1$ or $\mD = \mD_2$ with probability at least $\frac23$, giving the lemma.
%
%To ensure that \(\tilde\trace(\mM)\) can distinguish the two cases, we need to ensure that the upper bound for \(\tilde\trace(\mG^T\mD_1\mG)\) is strictly below the lower bound for \(\tilde\trace(\mG^T\mD_2\mG)\), which happens when \(d \geq \frac{6+3\eps-\eps^2}{\eps(1-\eps)}\).
%So, for large enough \(d\), the following algorithm differentiates \(\mD_1\) from \(\mD_2\) with probability \(\frac23\):
%\begin{center}
%	If \(\tilde\trace(\mM) \leq (1+\tsfrac\eps3)\cdot d \cdot (1+\tsfrac{6\ln(6\cdot24)}{d})\trace(\mD_1)\), return \(\mD_1\). Else, return \(\mD_2\).
%\end{center}
\end{proof}

We show that \problemref{trace-style} requires $\Omega(1/\epsilon)$ queries, which combined with \lemmaref{lower-bound-trace-style} proves our main lower bound, \theoremref{intro_lowerbound}, showing that \hutchppna is optimal for non-adaptive trace estimation. 

\subsection{Transforming \problemref{trace-style}}
We start by showing that for \problemref{trace-style} the user's non-adaptive queries might as well be the first $m$ standard basis vectors.
%
%\theoremref{lower-bound} proves that \hutchpp has an optimal query complexity amongst non-adaptive algorithms, and is proved by a series of WLOG arguments that reduce \problemref{trace-style} down to the problem of distinguishing \(\chi^2\) random variables.
%Before diving into the main reductions, note that without loss of generality the \emph{user only sends orthonormal queries} (i.e. \!\mU is orthogonal), which holds because the matrix-vector oracle is linear.

%\subsection{Removing the Query}
\begin{lemma}
\label{lem:remove-query}
In \problemref{trace-style}, without loss of generality, the user just submits query matrix \(\mU = \mE_m=\bmat{\ve_1 & \ldots & \ve_m}\), the first \(m\) standard basis vectors.
\end{lemma}
\begin{proof}
First note that we can assume without loss of generality that the query matrix $\mU$ is orthonormal, since if it were not, we could simply reconstruct the queries $\mA \mU$ by querying $\mA$ with an orthonormal basis for the columns of $\mU$. 

Next, note that by the rotational invariance of the Gaussian distribution, if \(\mG \in \R^{d \times d}\) is an \iid \(\cN(0,1)\) matrix, and \(\mQ \in \R^{d \times d}\) is any orthogonal matrix, then \(\mG\mQ\) is  distributed identically to $\mG$.
Let  \(\bar\mU \in \R^{d \times d - m}\) be any orthonormal span for the nullspace of \mU, so that \(\mQ\defeq\bmat{\mU & \bar\mU}\) is orthogonal.
We have that  \(\mQ \cdot\mG^T\mD\mG \mE_m\) is distributed identically to \(\mQ \cdot  \mQ^T \mG^T\mD\mG \mQ \mE_m = \mG^T\mD\mG \mU\).
%So, since \(\mQ\mE_m = \mU\), we know that \(\mQ^T\mG^T\mD\mG\mE_m\) is distributed as \(\mG^T\mD\mG\mU\).
So, of the  user is forced to submit \(\mE_m\) as their query, and observe \(\mM = \mG^T\mD\mG\mE_m\), they can compute \(\mQ\mM\) and use that matrix instead, as it will follow the exact same distribution as if they submitted \mU in the first place and observed $ \mG^T\mD\mG \mU$.
\end{proof}

%\subsection{A Rotation on the Left}
%Now that we have removed the user's choice of query from \problemref{trace-style}, 
We next perform a transformation to remove one of the $\mG$ matrices from the matrix \(\mG^T\mD\mG\) in \problemref{trace-style}, to avoid complex 
%Since \mG appears twice in \(\mG^T\mD\mG\), this creates a 
correlations between the entries of \(\mG^T\mD\mG\) which make it hard to directly prove a statistical lower bound. We define the intermediate problem:
%Instead, we create something roughly like a random factorization of \(\mG^T\mD\mG\)
\begin{problem}
\label{prob:statistical-estimation}
Nature samples \(\mD=\mD_1\) or \(\mD=\mD_2\) with equal probability, \(\mG\in\bbR^{d \times m}\) with \iid \(\cN(0,1)\) entries, and uniform random orthogonal matrix \(\mZ\in\bbR^{d \times d}\).
The user observes \(\mZ\mD\mG\) and guesses if \(\mD=\mD_1\) or \(\mD=\mD_2\).
\end{problem}
\begin{lemma}
\label{lem:reduce-to-statistical-estimation}
Let \cA be an algorithm capable of solving \problemref{trace-style}.
Then \cA can be used to solve \problemref{statistical-estimation} with the same success probability.
\end{lemma}
\begin{proof}
By \lemmaref{remove-query}, we just need show how to use the observed matrix \(\mN = \mZ\mD\mG\) in \problemref{statistical-estimation}  to create a sample from the distribution \(\hat\mG^T\mD\hat\mG \mE_m\) where $\hat \mG \in \R^{d \times d}$ has \iid \(\cN(0,1)\) entries.
%Note that \(\mG\in\bbR^{d \times k}\) for \problemref{statistical-estimation}, but \(\hat\mG\in\bbR^{d \times d}\) for \problemref{trace-style}.
%Let \(\mN \defeq \mZ\mD\mG\) be the observed matrix.
To do this,
%In order to generate a samples from \(\hat\mG^T\mD\hat\mG\), 
we sample \(\mL\in\bbR^{d \times (d-k)}\) with \iid \(\cN(0,1)\) entries, and compute:
\[
	\mM = \bmat{\mN^T\mN \\ \mL^T\mN}.
\]
%To see that \(\mM\) is distributed as \(\hat\mG^T\mD\hat\mG \mE_m\) where $\hat \mG \in \R^{d \times d}$ has \iid \(\cN(0,1)\) entries, 
First note that \(\mN^T\mN = \mG^T\mD^T\mZ^T\mZ\mD\mG = \mG^T\mD\mG \in \bbR^{m \times m}\).
Next, observe that \(\tilde\mG^T\defeq\mL^T\mZ\) has i.i.d. \(\cN(0,1)\) entries since \mZ is orthogonal, and is  independent of $\mG$. $\mL^T \mN = \tilde\mG^T\mD\mG\) and overall:% has i.i.d. \(\cN(0,1)\) entries and is independent of $\mG$.
\[
	\mM
	= \bmat{\mN^T\mN \\ \mL^T\mN}
	= \bmat{\mG^T\mD\mG \\ \tilde\mG^T\mD\mG}
	= \bmat{\mG ~ \tilde\mG}^T\mD\mG
	= \hat\mG^T\mD\hat\mG\mE_m,
\]
where \(\hat\mG\defeq\bmat{\mG ~ \tilde\mG} \in \R^{d \times d}\) has i.i.d. \(\cN(0,1)\) entries.
% in \(\bbR^{d \times d}\), \(\mM\) must be distributed as in \problemref{trace-style} with query matrix \(\mE_m\). 
Thus $\mM$ is distributed as in \problemref{trace-style} with query matrix \(\mE_m\).% and so any algorithm solving \problemref{trace-style} can solve \problemref{statistical-estimation} with the same success probability.
\end{proof}

\subsection{Reduction to Hypothesis Testing}
Finally, we directly prove a lower bound on the statistical complexity of differentiating \(\mD_1\) and \(\mD_2\) in \problemref{statistical-estimation}, and thus, via \lemmaref{reduce-to-statistical-estimation}, \problemref{trace-style}
\begin{lemma}
\label{lem:statistical-lower-bound}
If \(m < \frac{2}{9\eps}\), then \problemref{statistical-estimation}, and thus \problemref{trace-style} cannot be solved with probability \(\ge \frac23\).
\end{lemma}

Combined with \lemmaref{lower-bound-trace-style}, this immediately yields our main lower bound on non-adaptive trace estimation, \theoremref{intro_lowerbound}.
%\label{thm:lower-bound}
%Any non-adaptive algorithm requires at least \(\frac{\ln(\nicefrac43)}\eps\) queries to solve \problemref{trace-style} with probability \(\frac23\).
%\end{theorem}

\begin{proof}
Let $\cP$ be the distribution of $\mZ \mD\mG$ in \problemref{statistical-estimation}, conditioned on $\mD = \mD_1$, and let $\cQ$ be the distribution conditioned on $\mD = \mD_2$. We will show that when $m < \frac{2}{9\eps}$, the KL-divergence between these two distributions is bounded by $D_{KL}(\cP\|\cQ) \le \frac{2}{9}$. By Pinsker's inequality, this gives that the total variation distance is bounded by $TV(\cP,\cQ) \le \frac{1}{3}$, and thus no algorithm can solve \problemref{statistical-estimation} with probability $\ge \frac{2}{3}$.

%We will show for $m < BLAH$, the total variation distance $TV(\cP,\cQ)$ is upper bounded by $1/3$. In turn, no algorithm can solve \problemref{statistical-estimation} with probability $\ge \frac{2}{3}$. To do this, w


%By the Neyman-Pearson Lemma (Lemma 5.3 in \cite{rigollet2015high}) and Lemma 2.6 from \cite{DBLP:books/daglib/0035708}, we know that any classifier trying to distinguish a sample from distribution \cP and a sample from distribution \cQ fails with probability \(\frac13\) if \(\frac13 \geq \frac14 e^{-D_{KL}(\cP\|\cQ)}\).
%In our case, \(\cP\) is the distribution of generating \mZ and outputting \(\mZ\mD_1\mG\) and \(\cQ\) is the distribution of generating \mZ and outputting \(\mZ\mD_2\mG\).
%So, our goal is to upper bound the Kullback-Leibler divergence between these distributions.
%Since \cP and \cQ involve the process of sampling \mZ, we cannot apply a black-box bound for the KL Divergence of two Gaussians.
%Instead, we reparameterize \cP and \cQ until we can use more direct bounds.

First observe that \cP and \cQ are distributions on $d \times m$ matrices whose columns are drawn independently from   
%
%We start by focusing on \cP, associated with the rank-\(n\) \(\mD_1\) matrix.
%Consider the columns of \(\mZ\mD_1\mG\) as a sequence of \(k\) vectors in \(\bbR^d\) drawn from \
\(\cN(\vec0,\mZ\mD_1\mZ^T)\) and \(\cN(\vec0,\mZ\mD_2\mZ^T)\)  respectively. %, which are \iid conditioned on \mZ.
Equivalently, each column is drawn from a joint distribution over parameters in polar form: instead of the distribution over \(\vx\in\bbR^{d}\), consider the joint distribution of \((\normof\vx^2, \frac{\vx}{\normof\vx})\in(\bbR \times \cB_d)\) where \(\cB_d\) is the unit ball in \(d\) dimensions.
Let \(\cM_{\cP, \mZ}\) and \(\cM_{\cQ, \mZ}\) be the distributions over the columns' squared magnitudes conditioned on $\mZ$ and \(\cD_{\cP,\normof\vx}\) and \(\cD_{\cQ,\normof\vx}\) be the distributions over directions, conditioned on \(\normof\vx\).
Since \(\cN(\vec0,\mZ\mD_1\mZ^T)\) and  \(\cN(\vec0,\mZ\mD_2\mZ^T)\)  are rank-\(n\) and rank-$(n+1)$ isotropic Gaussians respectively, and since $\mZ$ is orthogonal, \(\cM_{\cP, \mZ}\) and \(\cM_{\cQ, \mZ}\) are chi-squared distributions with $n$ and $n+1$ degrees of freedom respectively. I.e., $\cM_{\cP, \mZ} = \chi_{n}^2$ and $\cM_{\cQ, \mZ} = \chi_{n+1}^2$.
%
%each column vector has square L2 norm distributed as a \(\chi^2\) random variable: \(\cM_{\mZ} = \chi_{k}^2\) no matter the value of \mZ.
Further, since \mZ is a {uniformly} random rotation matrix, 
%
%in both cases, the distribution of directions is independent of the norm of the column, and since %: \(\cD_{\mZ,\normof\vx} = \cD_{\mZ}\).
%\mZ is a {uniformly} random rotation matrix, 
%as long as the number of columns $m < n$, 
 %\(m \leq \rank(\mZ\mD_1\mZ^T) = n = \frac1\eps\), 
 both \(\cD_{\cP,\normof\vx}\) and \(\cD_{\cQ,\normof\vx}\) are the uniform distribution over \(\cB_d\), denoted  $\bbU_{\cB_d}$.
So, \(\cP\) is equivalently parameterized as a distribution over \(k\) \iid \(\chi_n^2\) variables and \(k\) \iid uniform random unit vectors on \(\bbR^d\).
Similarly, \cQ is parameterized as a distribution over \(k\) \iid \(\chi_{n+1}^2\) variables and \(k\) \iid uniform random unit vectors.
Since Kullback-Leibler divergence is invariant over parameterizations and linear over independent samples \cite{kullback1951}, we find that:
\[
	D_{KL}(\cP\|\cQ) = m \cdot D_{KL}(\chi_n^2 \| \chi_{n+1}^2) + m  \cdot D_{KL}(\bbU_{\cB_d} \| \bbU_{\cB_d}) = m \cdot D_{KL}(\chi_n^2 \| \chi_{n+1}^2).
\]
%where \(\bbU_{\cB_d}\) is the uniform distribution over the unit ball \(\cB_d\).
%Since the KL Divergence from a distribution to itself is zero, \(D_{KL}(\bbU_{\cB_d} \| \bbU_{\cB_d})=0\), and so
%\[
%	D_{KL}(\cP\|\cQ) = m \cdot D_{KL}(\chi_n^2 \| \chi_{n+1}^2)
%\]
In \appendixref{dkl-bound}, we prove that \(D_{KL}(\chi_n^2 \| \chi_{n+1}^2) \leq \frac1n\).
Since \(n = \frac1\eps\), we find that
\[
	D_{KL}(\cP \| \cQ) \leq m\eps.
\]
Thus, if \(m \leq \frac{2}{9\eps}\), then $D_{KL}(\cP\|\cQ) \le \frac{2}{9}$, completing the proof.
\end{proof}
%\subsection{Putting it All Together}
%\begin{theorem}
%\label{thm:lower-bound}
%Any non-adaptive algorithm requires at least \(\frac{\ln(\nicefrac43)}\eps\) queries to solve \problemref{trace-style} with probability \(\frac23\).
%\end{theorem}
%\begin{proof}[Proof of \theoremref{lower-bound}.]
%\lemmaref{reduce-to-statistical-estimation} tells us that any non-adaptive algorithm capable of solving \problemref{trace-style} with \(k\) queries and probability \(\frac23\) is also capable of solving \problemref{statistical-estimation} with \(k\) queries and probability \(\frac23\).
%By, \lemmaref{statistical-lower-bound} it is not possible to solve \problemref{statistical-estimation} with \(m < \frac{\ln(\nicefrac43)}{\eps}\) queries.
%So, there does not exist a non-adaptive algorithm that solves \problemref{trace-style} with less that \(\Omega(\nicefrac1\eps)\) samples and succeeds with probability \(\frac23\).
%\end{proof}


==> nonadaptive-estimation-old.tex <==
\section{Non-Adaptive Trace Estimation using Streaming Sketches}
Unlike the Hutchinson Estimator, the AdaHutch Estimator is \emph{adaptive}: it uses the result of a subspace iteration step to compute the matrix \mP, which is then used by the Hutchinson subroutine.
This raises the following theoretical question: \emph{Is Adaptivity neccessary for an \(O(\frac1\eps)\) query complexity?}
By appealing to a result from the streaming literature, we show that \emph{adaptivity is not needed}.
Though, the adaptive algorithm experimentally performs better.

The key theoretical tool here comes from the streaming literature.
Specifically, Theorem \(4.7\) from \cite{DBLP:conf/stoc/ClarksonW09} shows that we can non-adaptively find a matrix \(\tilde\mA_k\) such that \(\normof{\mA-\tilde\mA_k}_F \leq 2\normof{\mA-\mA_k}_F\) with \(O(k \log(\nicefrac1\delta))\) Matrix-Vector queries.
With this in hand, we propose the \emph{Hutch++} estimator:

\begin{theorem}
\label{thm:hutchplusplus}
Let \(\tilde\mA_k \in \bbR^{d \times d}\) such that \(\normof{\mA-\tilde\mA_k}_F \leq 2\normof{\mA-\mA_k}_F\).
Then let
\[
	\hutchpp_{k,\ell} \defeq \trace(\tilde\mA_k) + \hutch_\ell(\mA-\tilde\mA_k)
\]
which can be evaluated in \(\ell\) Matrix-Vector queries to \mA.
If \(\delta\in (2e^{-\nicefrac\ell8}, 1)\), then with probability \(1-\delta\), we have
\[
	\abs{\hutchpp_{k,\ell} - \trace(\mA)} \leq O\big( {\textstyle \sqrt{\frac{\log(\nicefrac1\delta)}{k\ell}}}\big) \trace(\mA)
\]
In particular, if \(k = \ell = O(\frac{\sqrt{\log(\nicefrac1\delta)}}{\eps})\), then \(\hutchpp_{k,\ell}\) uses \(O(\frac{\sqrt{\log(\nicefrac1\delta)}}{\eps})\) queries to get a \((1\pm\eps)\) relative error guarantee.
\end{theorem}
Note that since creating the \(\tilde\mA_k\) matrix requires \(O(k \log(\nicefrac1\delta)) = O(\frac{\log(\nicefrac1\delta)}{\eps})\) Matrix-Vector queries, the complete algorithm below only requires \(O(\frac{\log(\nicefrac1\delta)}{\eps})\) queries:

\begin{algorithm}[H]
	\caption{\(\hutchpp\)}
	\label{alg:hutchplusplus}
	% 
	{\bfseries input}: Matrix-Vector oracle to PSD Matrix \(\mA\in\bbR^{d \times d}\). Number of queries \(k\) and \(\ell\) (\(k\) is a factor of 3). \\
	%
	{\bfseries output}: Approximate Trace of \mA
	% 
	% \phantom{aaaaaaaaaaaaaaaaaaaaaaaaaaaaaaa}
	% \vspace{-\baselineskip}
	% 
\begin{algorithmic}[1]
	\STATE Sample \(\mS\in\bbR^{d \times \frac{2k}3}\), \(\mR\in\bbR^{d \times \frac k3}\), and \(\mG\in\bbR^{d \times \ell}\) with \iid \(\cN(0,1)\) entries.
	\STATE Compute sketch matrix \(\tilde\mA_k = \mA\mR(\mS^\intercal\mA\mR)^{\dagger}(\mA\mS)^\intercal\)
	\STATE {\bfseries return} \(\hutchpp_{k,\ell} = \trace(\tilde\mA_k) + \frac1\ell \trace(\mG^\intercal\mA\mG) - \frac1\ell \trace(\mG^\intercal\tilde\mA_k\mG)\)
\end{algorithmic}
\end{algorithm}

\begin{proof}[Proof of \theoremref{hutchplusplus}.]
By linearity of trace,
\[
	\trace(\mA) = \trace(\tilde\mA_k) + \trace(\mA-\tilde\mA_k)
\]
So, by definition of the \(\hutchpp_{k,\ell}\) estimator, we have
\begin{align*}
	\abs{\hutchpp_{k,\ell}(\mA) - \trace(\mA)}
	&= \abs{\trace(\mA-\tilde\mA_k) - \hutch_\ell(\mA-\tilde\mA_k)} \\
	&\leq \tilde O(\tsfrac{1}{\sqrt\ell})\normof{\mA-\tilde\mA_k}_F \\
	&\leq \tilde O(\tsfrac{1}{\sqrt\ell})\cdot 2 \normof{\mA-\mA_k}_F \\
	&\leq \tilde O(\tsfrac{1}{\sqrt\ell})\cdot \tsfrac{2}{\sqrt k} \trace(\mA) \\
	&= \tilde O(\tsfrac{1}{\sqrt{k \ell}}) \trace(\mA) \\
\end{align*}
\end{proof}


==> nonadaptive-estimation.tex <==
\section{\texorpdfstring{\(\hutchpp\)}{Hutch++}: A Faster non-Adaptive Trace Estimator}
One of the benefits of the Hutchinson estimator is that it is \emph{non-adaptive}: all the matrix-vector queries can be computed in one large batch, and the trace estimate can be computed without using any more matrix-vector queries.
A result from the streaming literature, specifically Theorem 4.7 from \cite{DBLP:conf/stoc/ClarksonW09}, shows that \(O(k \log\nicefrac1\delta)\) matrix-vector queries suffices to find a matrix \(\tilde\mA_k\) such that \(\normof{\mA-\tilde\mA_k}_F \leq 2\normof{\mA-\mA_k}_F\).
With this in hand, we propose the \(\hutchpp\) estimator:
\begin{theorem}
Let \(\tilde\mA_k\in\bbR^{d \times d}\) such that \(\normof{\mA-\tilde\mA_k}_F \leq 2 \normof{\mA-\mA_k}_F\).
Then let
\begin{align}
\label{eq:hutchpp}
	\hutchpp_{k,\ell}(\mA) \defeq \trace(\tilde\mA_k) + \hutch_\ell(\mA-\tilde\mA_k)
\end{align}
which can be evaluated in \(\ell\) Matrix-Vector queries to \mA.
If \(\delta\in(0,1)\), then with probability \(1-\delta\), we have
\[
	\abslr{\hutchpp_{k,\ell}(\mA) - \trace(\mA)} \leq O\big(\sqrt{\tsfrac{\log(\nicefrac1\delta)}{k\ell}}\big) \trace(\mA)
\]
In particular, if \(k = \ell = O(\frac{\sqrt{\log(\nicefrac{1}{\delta})}}\eps)\), then \(\hutchpp_{k,\ell}(\mA)\) uses \(O\left(\frac{\sqrt{\log(\nicefrac1\delta)}}{\eps}\right)\) Matrix-Vector queries to achieve relative error \(\eps\) with probability \(1-\delta\).
\end{theorem}
\begin{proof}
By linearity of trace, note that
\[
	\trace(\mA) = \trace(\tilde\mA_k) + \trace(\mA-\tilde\mA_k)
\]
So, comparing to the definition of \(\hutchpp_{k,\ell}(\mA)\) in \equationref{hutchpp}, we have
\begin{align*}
	\abs{\hutchpp_{k,\ell}(\mA) - \trace(\mA)}
	&= \abs{\trace(\mA-\tilde\mA_k) - \hutch_\ell(\mA-\tilde\mA_k)} \\
	&\leq \tilde O(\tsfrac{1}{\sqrt{\ell}}) \normof{\mA-\tilde\mA_k}\\
	&\leq \tilde O(\tsfrac{1}{\sqrt{\ell}}) \cdot 2 \normof{\mA-\mA_k}\\
	&\leq \tilde O(\tsfrac{1}{\sqrt{\ell}}) \cdot \tsfrac{2}{\sqrt k} \trace(\mA)\\
	&= \tilde O(\tsfrac{1}{\sqrt{k\ell}}) \trace(\mA)
\end{align*}
\end{proof}
Note that since Theorem 4.7 from \cite{DBLP:conf/stoc/ClarksonW09} requires \(O(k \log\nicefrac1\delta)\) matrix-vector queries, the complete algorithm below requires \(O(\frac{\log(\nicefrac1\delta)}{\eps})\) queries:
\begin{algorithm}[H]
	\caption{\(\hutchpp\)}
	\label{alg:hutchplusplus}
	% 
	{\bfseries input}: Matrix-Vector oracle for PSD \(\mA\in\bbR^{d \times d}\). Number of queries \(k,\ell\) (\(k\) is a multiple of 3). \\
	%
	{\bfseries output}: Approximate Trace of \mA
	% 
	% \phantom{aaaaaaaaaaaaaaaaaaaaaaaaaaaaaaa}
	% \vspace{-\baselineskip}
	% 
\begin{algorithmic}[1]
	\STATE Sample \(\mS\in\bbR^{d \times \frac{2k}3}\), \(\mR\in\bbR^{d \times \frac k3}\), and \(\mG\in\bbR^{d \times \ell}\) with \iid \(\cN(0,1)\) entries.
	\STATE Compute sketch matrix \(\tilde\mA_k = \mA\mR(\mS^\intercal\mA\mR)^{\dagger}(\mA\mS)^\intercal\)
	\STATE {\bfseries return} \(\hutchpp_{\ell} = \trace(\tilde\mA_k) + \frac1\ell \trace(\mG^\intercal\mA\mG) - \frac1\ell \trace(\mG^\intercal\tilde\mA_k\mG)\)
\end{algorithmic}
\end{algorithm}


